Towards Deployment-Efficient Reinforcement Learning: Lower Bound and Optimality

Deployment efficiency is an important criterion for many real-world applications of reinforcement learning (RL). Despite the community's increasing interest, there lacks a formal theoretical formulation for the problem. In this paper, we propose such a formulation for deployment-efficient RL (DE-RL) from an "optimization with constraints" perspective: we are interested in exploring an MDP and obtaining a near-optimal policy within minimal \emph{deployment complexity}, whereas in each deployment the policy can sample a large batch of data. Using finite-horizon linear MDPs as a concrete structural model, we reveal the fundamental limit in achieving deployment efficiency by establishing information-theoretic lower bounds, and provide algorithms that achieve the optimal deployment efficiency. Moreover, our formulation for DE-RL is flexible and can serve as a building block for other practically relevant settings; we give "Safe DE-RL" and "Sample-Efficient DE-RL" as two examples, which may be worth future investigation.

==> WorkingOnLemma.tex <==
\begin{lemma}
    Consider matrices $X_1,...,X_t$, and $\Sigma_t=\sum_{k=1}^{t-1}NX_k$, and $\Sigma_{t, N'}=\sum_{k=1}^{t-1}N'X_k$
\end{lemma}
\begin{proof}
    Suppose $X_1,...,X_{t-1}$ are linear independent, i.e. there does not exists $\resolution_1,...\resolution_{t-1}$, such that $\sum_{k=1}^{t-1}\resolution_k X_k=O$.
    
    Suppose we have decomposition that $X_t=X_{t\perp}+X_{t\parallel}$, where $Tr(X_{t\perp}X_k)=0$ for arbitrary $k=1,...,t-1$ and there exists $\alpha_{t,k}$ for $k=1,...,t-1$ such that $X_{t\parallel}=\sum_{k=1}^{t-1}\alpha_{t,k}X_k$.

    Suppose $|Tr(\Sigma_{t-1,N'}^{-1}X_{t-1,\perp})| \geq \resolution$
    Besides, we also have:
    \begin{align*}
        \delta \leq Tr(\Sigma_t^{-1}X_t)\leq Tr(\Sigma_{t-1}^{-1}X_t) \leq 1,\quad Tr(\Sigma_{t,N'}^{-1}X_t)\leq 1,\quad Tr(\Sigma_{t-1,N'}^{-1}X_t)\leq 1,\quad\forall N' \geq 0
    \end{align*}
    Therefore, the following holds for arbitrary $N'$
    \begin{align*}
        Tr(\Sigma_{t,N'}^{-1}X_{t\parallel})-Tr(\Sigma_{t-1,N'}^{-1}X_{t\parallel})=&Tr\Big(\Sigma_{t,N'}^{-1}\big(\sum_{k=1}^{t-1}\alpha_{t,k}X_k\big)\Big)-Tr\Big(\Sigma_{t-1,N'}^{-1}\big(\sum_{k=1}^{t-1}\alpha_{t,k}X_k\big)\Big)\\
        =&\sum_{k=1}^{t-1}\alpha_{t,k}Tr(\Sigma_{t,N'}^{-1}X_k)-\sum_{k=1}^{t-2}\alpha_{t,k}Tr(\Sigma_{t-1,N'}^{-1}X_k)-\alpha_{t,t-1}Tr(\Sigma_{t-1,N'}^{-1}X_{t-1})-\alpha_{t,t-1}Tr(\Sigma_{t-1,N'}^{-1}X_{t-1})
    \end{align*}
    Therefore,
    \begin{align*}
        2 \geq \lim_{N'\rightarrow \infty}|Tr(\Sigma_{t,N'}^{-1}X_{t\parallel})-Tr(\Sigma_{t-1,N'}^{-1}X_{t\parallel})| = \lim_{N'\rightarrow \infty}|\alpha_{t,t-1}Tr(\Sigma_{t-1,N'}^{-1}X_{t-1})| \geq \alpha_{t,t-1}\resolution
    \end{align*}
    Therefore,
    \begin{align*}
        |\alpha_{t,t-1}| \leq \frac{2}{\resolution}
    \end{align*}
    Besides, we can show that for arbitrary $k=1,2,...,t-1$,
    \begin{align*}
        \sum_{i=k}^{t-1}|\alpha_{t,t-1}|\leq \frac{2}{\resolution}
    \end{align*}
    Therefore, we can choose $N$ large enough such that,
    \begin{align*}
        |Tr(\Sigma^{-1}_tX_{t\perp})| \geq \delta - O(\frac{1}{N}),\quad |Tr(\Sigma^{-1}_{k}X_{t\perp[1:k-1]})| \geq \delta - O(\frac{1}{N})
    \end{align*}
\end{proof}


\begin{lemma}
    We can show that, as long as $N\geq O(\frac{1}{\delta})$ and $Tr(\Sigma_t^{-1}X_t)\geq \delta$ at step $t$, we must have:
    \begin{align*}
        Tr(\Sigma_t^{-1}X_{t\perp [1:t-1]}) > 0
    \end{align*}
\end{lemma}
\begin{proof}
    Given matrices $X_1,...,X_t$.
    Denote $X_{k, \perp j}=X_k-\frac{Tr(X_kX_j)}{Tr(X_jX_j)}X_j$ satisfying that $Tr(X_{k, \perp j}X_j)=0$. Denote $X_{k, \perp [1:k-1]}$ as the component of $X_k$ orthogonal to the space spanned by $X_1,...,X_{k-1}$
    
    First of all,
    \begin{align*}
        Tr(\Sigma^{-1}_2 X_{2\perp 1}) =& Tr\Big(\Sigma^{-1}_2 \big(X_2-\frac{Tr(X_2X_1)}{Tr(X_1X_1)}X_1\big)\Big)\\
        =&Tr(\Sigma^{-1}_2 X_2)-\frac{Tr(X_2X_1)}{Tr(X_1X_1)} Tr(\Sigma^{-1}_2 X_1\big)\\
        \geq&\delta-\frac{d}{c^2(1+N)}
    \end{align*}
    and for arbitrary $X_k$ with $k\geq 2$, we have:
    \begin{align*}
        Tr(\Sigma^{-1}_2 X_{k\perp 1}) =& Tr\Big(\Sigma^{-1}_2 \big(X_k-\frac{Tr(X_kX_1)}{Tr(X_1X_1)}X_1\big)\Big)\\
        \leq&Tr\Big(\Sigma^{-1}_2 \big(X_2-\frac{Tr(X_kX_1)}{Tr(X_1X_1)}X_1\big)\Big)\\
        \leq&Tr(\Sigma^{-1}_2X_2)-\frac{c}{d+N} \tag{\red{check more}}\\
        =&Tr(\Sigma^{-1}_2 X_{2\perp 1})-O(\frac{1}{N})
    \end{align*}
    meanwhile,
    \begin{align*}
        Tr(\Sigma_2^{-1}X_{k\perp 1})=&Tr\Big(\Sigma^{-1}_2 \big(X_k-\frac{Tr(X_kX_1)}{Tr(X_1X_1)}X_1\big)\Big)\\
        \geq& Tr(\Sigma^{-1}_k X_k)-\frac{d}{c^2(1+N)}\\
        \geq& \delta-O(\frac{1}{N})
    \end{align*}
    Next, we consider $Tr(\Sigma^{-1}_3 X_{k\perp [1:2]})$.
    \begin{align*}
        Tr(\Sigma^{-1}_3 X_{k\perp [1:2]}) =& Tr(\Sigma^{-1}_3 X_k)-Tr(\Sigma^{-1}_3 X_{k\parallel [1:2]})\\
        \geq& Tr(\Sigma^{-1}_k X_k)-Tr(\Sigma^{-1}_3 X_{k\parallel [1:2]}) \\
        \geq& \delta - Tr(\Sigma^{-1}_3 X_{k\parallel [1:2]})\\
        \geq& \delta - Tr(\Sigma^{-1}_3 X_{k\parallel [1:2]\perp 1})-Tr(\Sigma^{-1}_3 X_{k\parallel [1:2]\parallel 1})
    \end{align*}
\end{proof}

\begin{proof}
    We start with $t=2$. Suppose we have $Tr\Big(\Sigma_2^{-1}X_2\Big) \geq \delta$. We define 
    $$
    \alpha_{2,1}=\arg\min_\alpha |Tr\Big(X_2 - \alpha X_1\Big)|,\quad s.t.\quad X_2 - \alpha X_1 \succeq 0,~\alpha > 0,
    $$
    Obviously, $\alpha_{2,1} \geq 0$, and we have:
    \begin{align*}
        \delta\leq Tr\Big(\Sigma_2^{-1}X_2\Big) =& \alpha_{2,1} Tr\Big(\Sigma_2^{-1}X_1\Big)+Tr\Big(\Sigma_2^{-1}\big(X_2 -\alpha_{2,1} X_1\big)\Big)\\
        \leq& \alpha_{2,1}\frac{\lambda d}{1+\lambda N}+Tr\Big(\Sigma_2^{-1}\big(X_2 -\alpha_{2,1} X_1\big)\Big)
    \end{align*}
    Since $X_2 - \alpha_{2,1} X_1 \succeq 0$, we have 
    \begin{align*}
        0 \leq Tr\Big(X_2 - \alpha_{2,1} X_1\Big) \leq 1 - \alpha_{2,1} Tr(X_1) \leq 1 - c \alpha_{2,1}
    \end{align*}
    Therefore, $\alpha_{2,1}\leq 1/c$, and we have
    \begin{align*}
        Tr\Big(\Sigma_2^{-1}\big(X_2 -\alpha_{2,1} X_1\big)\Big) \geq \delta - \alpha_{2,1}\frac{\lambda d}{1+\lambda N} \geq \delta - \frac{\lambda d}{c(1+\lambda N)} > 0
    \end{align*}
    As a result, we know that there does not exists $\resolution > 0$, such that $X_2 = \resolution X_1$, (in another word, $X_1$ and $X_2$ are independent). Otherwise, $Tr\Big(\Sigma_2^{-1}\big(X_2 -\alpha_{2,1} X_1\big)\Big) = 0$.

    Next, we do the induction at step $t$ with the starting condition that $\forall k \in[t]$, $Tr\Big(\Sigma_k^{-1}X_k\Big) \geq \delta$ and there does not exists $\resolution_1,...,\resolution_t \neq 0$ such that $\sum_{k=1}^{t-1}\resolution_k X_k = 0$. We define:
    \begin{align*}
        \alpha_{t,k}=\arg\max_\alpha X_t - \sum_{i=1}^{k-1} \alpha_{t,i}X_i-\alpha X_k,\quad s.t. X_t - \sum_{i=1}^{k-1} X_i-\alpha X_k \succeq 0\\
        \alpha_{t,1}...,\alpha_{t,t-1}=\arg\min_{\alpha_1,...,\alpha_{t-1}} Tr\Big(X_t - \sum_{i=1}^{t-1} \alpha_{i}X_i\Big),\quad s.t. X_t - \sum_{i=1}^{t-1} X_i\succeq 0,~\alpha_i \geq 0,\forall i\in[t]\\
    \end{align*}
    According to the definition, we have $\alpha_{t,k} \geq 0$ and $X_t - \sum_{k=1}^{t-1} \alpha_{t,k}X_k\succeq 0$, and therefore,
    \begin{align*}
        0 \leq Tr\Big(X_t - \sum_{k=1}^{t-1} \alpha_{t,k}X_k\Big)\leq 1-c\sum_{k=1}^{t-1} \alpha_{t,k}
    \end{align*}
    which implies that $\sum_{k=1}^{t-1} \alpha_{t,k}\leq 1/c$. Then, we have,
    \begin{align*}
        \delta \leq Tr\Big(\Sigma_t^{-1}X_t\Big)=&Tr\Big(\Sigma_t^{-1}\big(X_t-\sum_{k=1}^{t-1}\alpha_{k,t} X_k\big)\Big)+\sum_{k=1}^{t-1}\alpha_{k,t}Tr\Big(\Sigma_t^{-1} X_k\Big)\\
        \leq &Tr\Big(\Sigma_t^{-1}\big(X_t-\sum_{k=1}^{t-1}\alpha_{k,t} X_k\big)\Big)+\sum_{k=1}^{t-1}\alpha_{k,t} \frac{\lambda d}{1+\lambda N}\\
        \leq&Tr\Big(\Sigma_t^{-1}\big(X_t-\sum_{k=1}^{t-1}\alpha_{k,t} X_k\big)\Big)+\frac{\lambda d}{c(1+\lambda N)}
    \end{align*}
    which means that,
    \begin{align*}
        Tr\Big(\Sigma_t^{-1}\big(X_t-\sum_{k=1}^{t-1}\alpha_{k,t} X_k\big)\Big) \geq \delta - \frac{\lambda d}{c(1+\lambda N)} \geq 0
    \end{align*}
    Therefore, 
\end{proof}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\resolution$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\resolution{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

